Video Test-Time Adaptation for Action Recognition

Although action recognition systems can achieve top performance when evaluated on in-distribution test points, they are vulnerable to unanticipated distribution shifts in test data. However, test-time adaptation of video action recognition models against common distribution shifts has so far not been demonstrated. We propose to address this problem with an approach tailored to spatio-temporal models that is capable of adaptation on a single video sample at a step. It consists in a feature distribution alignment technique that aligns online estimates of test set statistics towards the training statistics. We further enforce prediction consistency over temporally augmented views of the same test video sample. Evaluations on three benchmark action recognition datasets show that our proposed technique is architecture-agnostic and able to significantly boost the performance on both, the state of the art convolutional architecture TANet and the Video Swin Transformer. Our proposed method demonstrates a substantial performance gain over existing test-time adaptation approaches in both evaluations of a single distribution shift and the challenging case of random distribution shifts. Code will be available at \url{https://github.com/wlin-at/ViTTA}.

==> fig/result_perCorruption.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{imgs/corruption_wise_acc.pdf}
\caption{
\label{fig:resultsCorruptionWise}
Corruption wise acc TANet UCF.
}
\end{figure*}



==> fig/teaser.tex <==
\begin{figure*}
\includegraphics[width=0.9\columnwidth]{imgs/teaser_two_column.pdf}
\caption{
\label{fig:teaser}
% Our online test-time video adaptation technique. The test videos are received singly. 
\wei{TODO change the caption}
Our test-time adaptation technique for video action recognition (\OurMethod) allows to adapt to distribution changes in a fully online manner, \ie processing each test video only once. 
% We perform inference right after adapting to a sample for one step. For the online test-time adaptation driven by feature distribution alignment, we adapt the model by pushing the statistics of the shifted test data towards that of the training data. 
Our architecture-agnostic \OurMethod aligns the statistics of test data towards the training data. 
After adaptation, the test data are more closely aligned with training data (bottom-right t-SNE~\cite{van2008visualizing} of mean features from final feature extractor layer for clean training data and 12 differently corrupted test datasets). The adaptation leads to a significant performance improvement for action recognition. 
% We plot the t-SNE~\cite{van2008visualizing} visualizations of mean features (from the last encoder layer) of training data, and of test data for 12 corruption types. Before adaptation, the shifted test data have statistics far away from the training data. After adaptation, the test data are more closely aligned with the training data, leading to performance improvement in action recognition.
 }
\end{figure*}


==> old_tex/intro.tex <==
\section{Introduction}

Motivation\\
\textbf{Motivation of Test time adaptation on video recognition: }\\
1. TO BE rephrased... since online adaptation does not require additional module parameters, it increases the portability on multiple devices and its access to diverse users. \\
2. as test data is not required to be stored, it respests privacy concerns. This is also of great importance on user videos with human actions. \\
3. as test data is not required to be stored, we do not need a large device for saving the video data. This is meaningful ful space-hungary data like video and point clouds. \\

motivation of the source-free setting: Traditional UDA methods require labeled source data and unlabeled target data. "Revisiting training data at test time can be impractical due to increasing privacy concerns, inflating sizes of datasets as well as many other real-world constraints".

\textbf{We compute source statistics:}: \\
source statistics do not violate the motivation of the source-free setting as\\
1) providing source statistics do not reveal the privacy of the raw source data, do not violate the data protection policy\\
2) source statistics are light-weight, and cause no burden of data transmission and data storage in comparison to the large amount of raw source data. \\
3) the computed source statistics are applicable on all types of model architectures, including CNN and transformer with only Laynorm with batch norm statistics. 


emphasize:\\
1) we do not use the ground truth label of test data. \\
2) mention the difference between video data and image data. In TTT, it says that "Batch normalization is ineffective when training with small batches, for which the estimated batch statistics are not accurate. This technically hurts TTT since each batch only contains (augmented) copies of a single image." But one video that contain a large number of frames is more informative, and we can compute more accurate statistics out of it, even with a small batch size\\

Introduction of corruption types on videos, application of test time adaptation for video recognition \\
apart from the corruption type that depend on content in a single image, we also cover temporal corruption types (e.g. packet loss in the video stream can propagate erros to consequent frames)

it is mentioned in the benchmark paper that "training models with noise or corruption degrades generalization and corruption robustness in video classification, while noise or corruption data augmentation play an important role in improving the robustness of image classification models. "

Online test time adaptation, the test data come in a sequential manner, each test sample is used only once\\

test time adaptation adapts at test time.  unlike test time training, \textbf{we do not required to alter the training condition by adding auxiliary task. 
The model only needs to be trained on the task of interest. (We only require the prior statistics from the already trained source model.) } \\
"the study seeks to answer the following question: how can we improve the robustness of ViT without retraining it from scratch? Most prior works focused on how to robustify the models during training. ... for example.. "\\
"TTA has two major advantages over usual training-time techniques:\\
first, it does not alter the training phase and thus does not need to repeat the computationally heavy training phase. Second, it does not require access to the source data during adaptation, which is impossible in the case of large pre-trained model."\\
"It is worth noting that the feature alignment approach for test-time adaptation (CFA and TTT++) assumes that one can access to the statistics on the source dataset during the test phase but does not need to access the source dataset itself and to repeat the computationally heavy training. \textbf{TTA generally assumes that the model would be distributed without source data due to bandwidth, privacy, or profit reasons. We argue that the statistics of source data would be distributed even in such a situation since it could drastically compress data size and elimiate sensitive information. In fact, some layers often used in typical neural networks contain statistics of source data (e.g. batch normalization)}. Therefore, this approach can be used without source dataset" 



Some selling points:\\
The approach is model-agnostic, we have evaluations on architectures of 2D+temporal module and Transformer. Transformer has Group Normalization layer instead of Batch normalization layer. "BN has been shown to be ineffective when training with small batches, for which the estimated batch statistics are not accurate"\\
Our method works \textbf{without elaborate selection of modulation parameters}. We update the parameters of the entire model. \\
Random frame sampling for two augmented views, video-specific contribution\\
alignment of two target views with source statistics lead to more adaptation info, this takes full advantage of the prior statistics that we pre-compute. Note that test data come in a sequential manner, each test sample is used only once\\
Minor: the prediction consistency regularization between two augmented views (after the classifier). \\
we can reach batch size of 1 for real online application, we outperform the baseline by a large margin using batch size of 1. This facilitates the application in real online adaptation where the video comes in one at a time. There is no need to collect a batch of videos before feeding the model. 




==> tex/abstract_modified_byhilde.tex <==
\begin{abstract}
Although action recognition systems can achieve top performance when evaluated on in-distribution test points, they are vulnerable to unanticipated distribution shifts in test data. The task of test-time adaptation, thus the adaption to corruptions during inference, has been proposed to provide a remedy in case of images. We follow this idea and propose to address the problem of video test-time adaptation with an approach tailored to spatio-temporal models that is capable of adapting on a single video sample at a step. It consists in a feature distribution alignment technique that aligns the test set statistics towards the original training statistics in as online manner. We further enforce prediction consistency over temporally augmented views of the same test video sample. Our method is is architecture-agnostic and can be integrated in various the state of the art convolutional and transformer architecture. 
Evaluations on three benchmark action recognition datasets show that the proposed technique 
%oblivious of network architecture, 
%and able to significantly boost the performance
%Our proposed method 
demonstrates a substantial performance gain over existing test-time adaptation approaches in both evaluations of single distribution shift and the challenging case of random distribution shift.
\end{abstract}


==> tex/defs.tex <==
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\newcommand{\net}{\phi}
\newcommand{\inpt}{\mathbf{x}}
\newcommand{\TrSet}{\mathit{S}}
\newcommand{\TeSet}{\mathit{T}}
\newcommand{\param}{\mathbf{\theta}}
\newcommand{\optParam}{\hat{\param}}

\newcommand{\mean}{\mu}
\newcommand{\var}{\sigma^2}
\newcommand{\trmean}{\hat{\mu}}
\newcommand{\trvar}{\hat{\sigma}^2}

\newcommand{\layer}{l}
\newcommand{\Layers}{L}
\newcommand{\voxel}{v}
\newcommand{\Voxels}{V}
\newcommand{\nchannels}{c_\layer}
\newcommand{\nframes}{t_\layer}
\newcommand{\height}{h_\layer}
\newcommand{\width}{w_\layer}
\newcommand{\voxelrange}{[1,\nframes]\times[1,\height]\times[1,\width]}

\DeclareMathOperator{\EX}{\mathbb{E}}% expected value

\newcommand{\mycomment}[1]{}

\newcommand{\myparagraph}[1]{\vspace{2pt}\noindent{\bf #1}}

\newcommand{\OurMethod}{ViTTA\xspace}
% \def\OurMethod{{ViTTA}}



\newif\ifdraft
\draftfalse
\drafttrue % <---- The way to switch between draft mode is to comment this


\definecolor{orange}{rgb}{1,0.5,0}
\definecolor{violet}{RGB}{70,0,170}
\definecolor{magenta}{RGB}{170,0,170}
\definecolor{dgreen}{RGB}{0,150,0}

% Strikethrough
\usepackage[normalem]{ulem}

\ifdraft
 \newcommand{\Wei}[1]{{\color{blue}{\bf Wei: #1}}}
 \newcommand{\wei}[1]{{\color{blue} #1}}
 \newcommand{\MK}[1]{{\color{magenta}{\bf MK: #1}}}
 \newcommand{\mk}[1]{{\color{magenta} #1}}
\else
 \newcommand{\Wei}[1]{}
 \newcommand{\wei}[1]{#1}
 \newcommand{\MK}[1]{}
 \newcommand{\mk}[1]{#1}
\fi




==> tex/introduction.tex <==
\section{Introduction}

In many applications, action recognition systems can be exposed to unexpected changes in the imaging conditions and, in consequence, to unanticipated shifts in the distribution of the input data.
A traffic camera, for example, may register rare weather events, like a hailstorm.
Systems deployed at sports fields can be affected by perturbations generated by humans, like the smoke of flares, forbidden in sports arenas, but occasionally used by some spectators.
Shifts in the data distribution can also result from inconspicuous changes to the image acquisition setup, for example, a change of the algorithm used to compress the video feed.
Recent work suggests that such distribution shifts can be detrimental to the performance of action recognition systems~\cite{yi2021benchmarking,schiappa2022large}, and practice shows that failures may be provoked even by physical traits of people present in the scene~\cite{ballTrackingFailure}.

In the domain of image classification, distribution shift in test data was addressed by Test-Time-Adaptation (TTA)~\cite{wang2021tent,liang2020shot,iwasawa2021test,schneider2020norm,sun2020ttt,liu2021tttpp,mirza2022dua,kojima2022cfa}, which uses the unlabelled test data to adapt the classifier to the change in data distribution.
The main adaptation techniques include regularizing the classifier on test data with loss functions defined on the entropy of its predictions~\cite{wang2021tent,liang2020shot},
updating the statistics of the batch normalization layers to match the distribution of the test data~\cite{schneider2020norm,mirza2022dua},
and training the network on test data with self-supervised tasks~\cite{sun2020ttt,liu2021tttpp}.
To the best of our knowledge, test-time-adaptation of video recognition models has so far not been demonstrated. 
We show that methods developed for image classification do not perform well in practical, online action recognition scenarios.
The performance difference between these two tasks stems from the differences in respective setups.
Architectures used for action recognition in videos are typically more memory-hungry than image classification networks, because their feature maps have an additional dimension representing the temporal aspect of the data. 
This limits the size of test batches that can be used for adaptation and, in consequence, affects the efficacy of most existing TTA methods, designed to work on large data samples. 



We address the problem of test time adaptation of video recognition networks with an approach tailored to temporal models. It consists in a feature alignment technique capable of adaptation on batches \wei{?} as small as a single video sequence.
To that end, instead of aligning statistics of test batches to those of the training set, it maintains online estimates of test set statistics and aligns them with the statistics of the training data \wei{rephrase?}. 
To further boost performance, it leverages on the temporal dimension of the data, and enforces prediction consistency across re-sampled copies of the same test video sequence.
Our contributions can be summarized as follows.
\begin{itemize}[nosep,label={--}]
  \item We benchmark existing TTA techniques in video action recognition and highlight their failures.
  \item We adapt the distribution alignment approach to online action recognition, generating a substantial performance gain over previous techniques.
  \item We propose a novel adaptation method that enforces consistency of predictions for randomly \wei{not necessarily randomly sampled} re-sampled frame sequences and show that it contributes to adaptation efficacy. 
\end{itemize}
The proposed technique is oblivious of the network architecture. We show that it boosts performance of both TANet~\cite{liu2021tam}, the state of the art convolutional architecture, and the Video Swin Transformer~\cite{liu2022video}.
Thanks to its low computation and memory requirements, our method can be run on hardware typically used for inference, which facilitates its deployment in existing systems.
It is truly source-free and fully online. Training samples \wei{training samples or test samples?} are processed one-by-one and discarded, which ensures maximum privacy preservation both for training and test data.
It requires statistics of the training data, but we show that batch normalization statistics can be used in architectures equipped with BN layers, at a modest performance penalty. \wei{move bullet points of contributions to the end of introduction so that reviewers easily locate them? }

\wei{re-organize the last paragraph? Emphasize the motivation of 1) low computation and memory requirement for adaptation on protable device 2) privacy protection of test user videos 3) completely source-free, does not require training data for adaptation }

\wei{explain that video data are more informative than image data, online adaptation of batch size 1 is feasible? }

\wei{
In our evaluation, we do not constrain that the sequence of test data all come from the same test distribution. 
In case each single test sample comes from randomly chosen distribution, our system still learns to adapt to the samples.}

\wei{online test time adaptation, adapting to one sample at a time allows decent flexibility}

\wei{In this work, we focus on test time adaptation that makes no assumption about training procedure (no alteration on the training condition, as re-training large-scale spatio-temporal model could be cost intensive), which is broadly applicable at test time.}



==> tex/introduction_modified_by_hilde.tex <==
\section{Introduction}
State-of-the-art neural architectures~\cite{feichtenhofer2020x3d,wang2021action,yang2020temporal,xiang2022spatiotemporal,yang2022recurring,truong2022direcformer} are very effective in action recognition, but recent work shows they are not robust to shifts in the distribution of the test data~\cite{yi2021benchmarking,schiappa2022large}.
Unfortunately, in practical scenarios, such distribution shifts are very difficult to avoid, or account for.
For example, cameras used for recognizing motorized or pedestrian traffic events may register rare weather conditions, like a hailstorm,
and sports action recognition systems can be affected by perturbations generated by spectators at sports arenas, such as the smoke of flares.
Shifts in the data distribution can also result from inconspicuous changes in the video processing setup, for instance, a change of the algorithm used to compress the video feed.


% \input{fig/teaser}
\input{fig/teaser_single_column}
In image classification, distribution shift can be successfully mitigated by Test-Time-Adaptation (TTA)~\cite{wang2021tent,liang2020shot,iwasawa2021test,schneider2020norm,sun2020ttt,liu2021tttpp,mirza2022dua,kojima2022cfa}, which uses the unlabeled test data to adapt the model to the change in data distribution.
However, methods developed for image classification are not well suited for action recognition.
Most action recognition applications require running memory- and computation-hungry temporal models online, with minimal delay, and under tight hardware constraints.
Moreover, videos are more vulnerable to distribution shifts than images~\cite{yi2021benchmarking,schiappa2022large,azimi2022self}. Some examples of such distribution shifts are given in Fig.~\ref{fig:teaser}. 
Due to limited exposure times, video frames are likely to feature higher variations of noise level, provoked by illumination changes. 
They are more affected by motion blur, which varies with the speed of motion observed in the scene.
They also feature stronger compression artifacts, which change with the compression ratio, often dynamically adjusted to the available bandwidth.
Our experiments show that existing TTA algorithms, developed for image classification, do not cope with these challenges well, yielding marginal improvement over networks used on corrupted data without any adaptation.

In our setup we follow the protocol of image test-time adaptation. In this case, each test sample is only processed once, and the model is updated regularly after $n$ samples. After each update, the last batch is forwarded and classified. The final accuracy is thus not computed based on the finally trained network, but accumulated during test-time adaptation as the mean over all results while updating the network. 
%
% Our goal is to propose an effective method for online test-time-adaptation of action recognition models.
% Operating online and with small latency can require drastically constraining the batch size, especially when the hardware resources are limited and the employed model is large.
We therefore address this scenario in which test samples are processed individually, including the special case of a batch size of one, thus processing one video at a time.
To ease the integration of our method in existing systems, we require it to be capable of adapting previously trained networks, both convolutional and transformer-based, without the need to retrain them.

In the work, we propose the first video test-time adaptation approach - ViTTA. To address the above requirements, we turn to feature alignment~\cite{sun2016coral,zellinger2017central,schneider2020norm,mirza2022dua,kojima2022cfa}, a common TTA method that aligns distributions of features computed for test and training data by minimizing discrepancy between their statistics.
Feature alignment does not require any modifications to the training procedure and is architecture-agnostic.
However, existing feature alignment methods are not well suited for online adaptation, because they require relatively large test batches to accurately estimate the statistics.
% kojima2022cfa - batch size 64
% schneider2020norm - batch size 64 for good results on imagenet, etc
% mirza2020dua - batch size 8 enough for good results on cifar10c?
% liang2020shot - batch size 64
We address this by employing the exponential moving average to estimate test feature statistics online.
This enables us to perform the alignment by processing one video sample at a time, at a low computational and memory cost.
Additionally, we show that even though the temporal dimension of video data poses challenges, it also has a silver lining.
We leverage this by creating augmented views of the input videos via temporally resampling frames in the video. This has two benefits: First, multiple augmented views lead to more accurate statistics of the overall video content. Second, it allows us to enforce prediction consistency across the views, making the adaptation more effective.

Our extensive evaluations on three most popular action recognition benchmarks demonstrate that \OurMethod boosts the performance of both TANet~\cite{liu2021tam}, the state-of-the-art convolutional architecture, and the Video Swin Transformer~\cite{liu2022video}, and outperforms the existing TTA methods proposed for image data by a significant margin. \OurMethod performs favorably in both, evaluations of single distribution shift and the challenging case of random distribution shift. 

% \OurMethod also has a high practical valor.
% % It is fully online and introduces modest computational and memory overheads, which makes it applicable in use cases requiring minimal delays.
% It is fully online and applicable in use cases requiring minimal delays. It does not require collection or storage of test video dataset, which is significant in terms of data privacy protection, especially in processing confidential user videos.
% \OurMethod can be seamlessly incorporated in systems already in operation, as it has no requirement of re-training existing networks. Therefore it can harness state-of-the-art video architectures. 
% % It is truly source free. It requires statistics of the training data, but we show that little performance is sacrificed when they are substituted with statistics accumulated at the Batch Normalization layers, if the network has them. 

Our contributions can be summarized as follows:
\begin{itemize}[nosep] %,label={--}]
  \item We benchmark existing TTA methods in online adaptation of action recognition models to distribution shifts in test data, on three most popular action recognition datasets, UCF101~\cite{soomro2012ucf101}, Something-something v2~\cite{goyal2017something} and Kinetics 400~\cite{kay2017kinetics} 
  % and show that they yield little improvement over un-adapted models. 
  \item We adapt the feature alignment approach to online action recognition, generating a substantial performance gain over existing techniques.
  \item We propose a novel, video-specific adaptation technique (\OurMethod) that enforces consistency of predictions for temporally re-sampled frame sequences and show that it contributes to adaptation efficacy. 
\end{itemize}




==> tex/introduction_wei.tex <==
\section{Introduction}
The task of action recognition has seen tremendous success in recent years with advances in neural networks and large-scale datasets~\cite{feichtenhofer2020x3d,wang2021action,yang2020temporal,xiang2022spatiotemporal,yang2022recurring,truong2022direcformer}. 
While achieving top performance on in-distribution test points, in reality, action recognition systems can be exposed to unanticipated shifts in the distribution of the test data. Such unexpected changes could be due to unstable conditions in the procedure of both video acquisition and video processing. A traffic camera, for example, may register rare weather events, like a hailstorm. Surveillance systems deployed at a sports field can be affected by perturbations generated by humans, such as the smoke of flares, prohibited in sports arenas, but occasionally used by some spectators. Shifts in the data distribution can also result from inconspicuous changes in the video processing setup, for instance, a change of the algorithm used to compress the video feed. 
%and practice shows that even a slightest shift in physical traits of humans present in the scene could provoke system perception failures~\cite{ballTrackingFailure}. 
\wei{to shorten, replace with video-specific examples}

In image classification, distribution shift in test data was addressed by Test-Time-Adaptation (TTA)~\cite{wang2021tent,liang2020shot,iwasawa2021test,schneider2020norm,sun2020ttt,liu2021tttpp,mirza2022dua,kojima2022cfa}, which uses the unlabeled test data to adapt the model to the change in data distribution.
The main adaptation techniques include regularizing the classifier on test data with loss functions defined on the entropy of its predictions~\cite{wang2021tent,liang2020shot},
updating the statistics of the batch normalization layers to match the distribution of the test data~\cite{schneider2020norm,mirza2022dua},
and training the network on test data with self-supervised tasks~\cite{sun2020ttt,liu2021tttpp,gandelsman2022test}. 

Video data, in comparison to images, are inherently more prone to distribution shifts. With the additional temporal dimension, there is an exponentially increasing space for unexpected changes in videos. Furthermore, as videos are in larger data amount, they are more easily exposed to quality degradation during processing such as high compression and high-speed transmission. Recent work suggests that such distribution shifts can be detrimental to the performance of action recognition systems~\cite{yi2021benchmarking,schiappa2022large}. 
However, to the best of our knowledge, test-time adaptation of video recognition models against common distribution shifts has so far not been demonstrated. 

In this work, we focus on a practical and challenging paradigm of video test-time adaptation. Specifically, given a model pretrained on clean training videos, we adapt it to potentially shifted unlabeled test videos that are received one by one in an online manner, without access to training data. 
We address this problem by leveraging an approach tailored to spatial-temporal models: First, we capture the mean and variance of the training distribution of the original model for each channel for multiple layers. At test time, we compute the same statistics of the test sample(s), assuming a distribution shift with respect to the training distribution. We then update the statistics of the parameters of the model based on the L1 loss between the trained model statistics and the new test distribution. The goal here is to adapt the model parameters so that they reproduce the training statistics even under corruptions in the test data. The training statistics thus serve as a form of ground truth that. the assumption is thus that the better those statistics can be reproduced under corruption, the better we can classify the test video. 
%
%
%It consists in a feature distribution alignment technique capable of adaptation on a single video sample at a step, as shown in Fig.~\ref{fig:teaser}. Specifically, we align the statistics of training data with that of test data. 
%Instead of computing test statistics on large batches, we maintain online estimates of test set statistics. 
% To this end, instead of aligning statistics of large test batches to those of the training set, it maintains online estimates of test set statistics and aligns them with the statistics of the training data \wei{rephrase?}. 
To further boost performance, we leverage on the temporal dimension of the data, and enforce prediction consistency across re-sampled views of the same test video sequence.

Note that in the proposed setting, test videos can be processed one-by-one without the need for long-term storage, which allows privacy preservation both for training and test data.
Additionally, if the pre-computed statistics of the training data are not available together with the pre-trained backbone, they can be generated from other data that follows the same underlying distribution, or as another option, the batch normalization statistics can be used, at least in case of architectures equipped with BN layers, at a modest performance penalty. The proposed method can be used in a source-free and/or online manner. 

Finally, our proposed technique generalizes across different the network architectures such as convolutional networks and transformers as long as they feature a spatial-temporal channel representation.


To evaluate the method, we propose a new benchmark setup for video test-time adaption. To this end, we leverage 3 popular video datasets, UCF101\cite{soomro2012ucf101}, Something-Something V2 \cite{goyal2017something}, and Kinetics-400\cite{kay2017kinetics}, and apply 12 different corruption types \hkc{if there are some nice corruptions in Fig 1 ref here} to the test data. We follow the protocol of image test-time adaptation \cite{whatever} and assume that the test data is received sequentially and that the network is updated regularly, and that inference is performed right after adaptation. We thus adapt to a sample or a set of samples and predict the class right after that. This process is repeated until each sample of the test set has been processed once. 

We show an evaluation of the proposed method on TANet~\cite{liu2021tam}, as a state-of-the-art convolutional architecture for action classification, and the Video Swin Transformer~\cite{liu2022video}. We compare the method in this challenging setup against state-of-the-art methods for image test-time-adaptation and show a significant performance gain. Moreover, we show that we are able to adapt the model not only to a single corruption type, as is standard in image test-time adaption, but the we can also handle various corruptions, as they may occur from different uploads to a video platform.



% Thanks to its low computation and memory requirements, our method can be run on hardware typically used for inference, which facilitates its deployment in existing systems. \hkc{Too applied!}




% Our motivations are:

% (1) We are interested in a model-agnostic adaptation approach that is oblivious of the network architecture and can harness any state-of-the-art video models.

% (2) We aim for a `plug-and-play' approach that requires neither additional modules upon the given model nor retraining with any auxiliary self-supervision task, to avoid the cost-intensive training phase on large-scale spatio-temporal backbones.  

% (3) The videos are received singly, and inference is performed right after adapting the model to a sample for one step. The model accumulates the knowledge of test videos in an online manner. In this case, it does not require collection of any test video dataset, which is significant in terms of data privacy protection, especially in processing private user videos. Moreover, as it neither stores space-hungry video dataset nor requires buffer for videos in large batches, this broadens application on portable devices. 

% In the practical online action recognition scenarios, we show that methods developed for image classification do not perform well.
% The performance difference between these two tasks stems from the differences in respective setups.
% Architectures used for video recognition are typically more memory-hungry than image networks, due to the additional temporal dimension in feature maps. 
% This limits the size of test batches that can be used for adaptation and, in consequence, affects the efficacy of most existing TTA methods, designed to work on large data batches.

\input{fig/teaser}



Our contributions can be summarized as follows.
\begin{itemize}[nosep,label={--}]
  \item We propose a video-tailored test-time adaptation method by a) adapting the distribution alignment approach to online action recognition and b) enforcing prediction consistency for re-sampled frame sequences.
  \item Our proposed method performs favorably in both evaluations of single distribution shift and the challenging case of random distribution shift, demonstrating a substantial performance gain over previous techniques. 
  \item We propose a new benchmark for video test-time adaptation based on the three most popular action recognition datasets, UCF101~\cite{soomro2012ucf101}, Something-something v2~\cite{goyal2017something} and Kinetics 400~\cite{kay2017kinetics}, with 12 image- and video-specific corruptions. 
  %and highlight their failures.
  % \item We propose a novel adaptation method that enforces consistency of predictions for re-sampled frame sequences and show that it contributes to adaptation efficacy. 
\end{itemize}


\wei{emphasizing the online/1-sample scenario in the introduction, highlighting the diffs between images and videos, and maybe incorporating some of your "advantages" that you listed at the end of the section}

% \wei{re-organize the last paragraph? Emphasize the motivation of 1) low computation and memory requirement for adaptation on protable device 2) privacy protection of test user videos 3) completely source-free, does not require training data for adaptation }

% \wei{explain that video data are more informative than image data, online adaptation of batch size 1 is feasible? }

\wei{
In our evaluation, we do not constrain that the sequence of test data all come from the same test distribution. 
In case each single test sample comes from randomly chosen distribution, our system still learns to adapt to the samples.}

\wei{online test time adaptation, adapting to one sample at a time allows decent flexibility}

\wei{In this work, we focus on test time adaptation that makes no assumption about training procedure (no alteration on the training condition, as re-training large-scale spatio-temporal model could be cost intensive), which is broadly applicable at test time.}
